Long Range Propagation on Continuous-Time Dynamic Graphs

Learning Continuous-Time Dynamic Graphs (C-TDGs) requires accurately modeling spatio-temporal information on streams of irregularly sampled events. While many methods have been proposed recently, we find that most message passing-, recurrent- or self-attention-based methods perform poorly on long-range tasks. These tasks require correlating information that occurred "far" away from the current event, either spatially (higher-order node information) or along the time dimension (events occurred in the past). To address long-range dependencies, we introduce Continuous-Time Graph Anti-Symmetric Network (CTAN). Grounded within the ordinary differential equations framework, our method is designed for efficient propagation of information. In this paper, we show how CTAN's (i) long-range modeling capabilities are substantiated by theoretical findings and how (ii) its empirical performance on synthetic long-range benchmarks and real-world benchmarks is superior to other methods. Our results motivate CTAN's ability to propagate long-range information in C-TDGs as well as the inclusion of long-range tasks as part of temporal graph models evaluation.

==> sections/CT-ADGN_1feb2024.tex <==
\section{\fulladgn}\label{sec:ctan}
Learning the dynamics of a C-TDG can be cast as the problem of learning information propagation following newly observed events in the system. This entails learning a diffusion function that updates the state of node $u$ as 
\vspace{-0.25mm}
\begin{equation}\label{eq:propagation}
\mathbf{h}_u(t) = F\left(t, \mathbf{x}_u, \mathbf{h}_u(t), \{\mathbf{h}_v(t)\}, \{\mathbf{e}_{uvt^-}\}\right),
\end{equation}
with $(v,t^-)\in\mathcal{N}^t_u$, and $\mathcal{N}^t_u = \{(v, t^-) \, |\,  \{u,v,t^-\} \in \mathcal{E}(t) \}$ is the temporal neighborhood of a node $u$ at time $t$, which consists of all the historical neighbors of $u$ prior to current time $t$. In the following, we omit the time subscript from the edge feature vector to enhance readability, since it refers to a time in the past in which the edge appeared. 

In recent literature, Eq.~\ref{eq:propagation} is modeled through a dynamical system described by a learnable ordinary differential equation (ODE)~\citep{GDE, grand, pde-gcn, graphcon, gravina2023antisymmetric}. Differently from discrete models, neural-ODE-based approaches learn more effective latent dynamics and have shown the ability to learn complex temporal patterns from irregularly sampled timestamps \citep{NeuralODE, ode-irregular, neuralCDE}, making them more suitable to address C-TDG problems.

In this paper, we leverage non-dissipative ODEs~\citep{StableArchitecture, AntisymmetricRNN, gravina2023antisymmetric} for the processing of C-TDGs. Thus, we propose a framework as a solution to a \textit{stable} and \textit{non-dissipative} ODE over a streamed graph. The main goal of our work is therefore achieving preservation of long-range information between nodes over a stream of events. We do so by first showing how a generic ODE can learn the hidden dynamics of a C-TDG and then by deriving the condition under which the ODE is constrained to the desired behavior.

First, we define a Cauchy problem in terms of the following node-wise ODE defined in time $t\in[0,T]$
\begin{small}
    \begin{equation}
\label{eq:ode}
    \frac{\partial\mathbf{h}_u(t)}{\partial t}=f_\theta\left(t, \mathbf{x}_u, \mathbf{h}_u(t), \{\mathbf{h}_v(t)\}_{v\in\mathcal{N}^t_u}, \{\mathbf{e}_{uv}\}_{v\in\mathcal{N}^t_u}\right)
\end{equation}
\end{small}
and subject to an initial condition $\mathbf{h}_u(0) \in \mathbb{R}^d$. The term $f_\theta$ is a function parametrized by the weights $\theta$ that describes the dynamics of node state. We observe that this framework can naturally deal with events that arrive at an arbitrary time. Indeed, the original Cauchy problem in Eq.~\ref{eq:ode} can be divided into multiple sub-problems, one per each event in the C-TDG.
The $i$-th sub-problem, defined in the interval $t\in[t_s, t_e]$, is responsible for propagating only the information encoded by the $i$-th event. Overall, when a new event $o_i$ happens, the ODE in Eq.~\ref{eq:ode} computes new nodes representations, $\mathbf{h}_u^i(t_e)$, starting from the initial configurations, $\mathbf{h}_u^i(t_s)$. In other words, $f_\theta$ evolves the state of each node given its initial condition. The top-right of Figure~\ref{fig:method} visually summarizes this concept, showing the nodes evolution given the propagation of an incoming event.
We observe that the knowledge of past events is preserved and propagated in the system thanks to an initial condition that includes not only the current node input states but also the node representations computed in the previous sub-problem, \ie $\mathbf{h}^i_u(t_s)=\psi(\mathbf{h}_u^{i-1}(t_e), \mathbf{x}_u(i))$. We notice that the terminal time $t_e$ is responsible for determining the extent of information propagation across the graph, since it limits the propagation to a constrained distance from the source. Consequently, smaller values of $t_e$ allow only for localized event propagation, whereas larger values enable the dissemination of information to a broader set of nodes.

\begin{figure*}[h]
\begin{center}
    %[trim={left bottom right top},clip]
    %\includegraphics[trim={0 0.8cm 0 1cm},clip,width=0.9\linewidth]{imgs/main_fig.png}
    \includegraphics[width=0.7\linewidth]{imgs/main_fig_v2.png}
\end{center}
\vspace{-4pt}
\caption{A high-level overview of the proposed framework illustrated for the $i$-th Cauchy sub-problem. On the left, we depict the propagation of the information of event $o_i$ through the graph. The faded portion of the graph corresponds to historical information, while the rest is the incoming event. On the right, we illustrate the evolution of node states given the propagation of the incoming event. Specifically, the top right shows the evolution as an ODE, $f_\theta$, that computes the node representation for a node $k$,  $\mathbf{h}_k(t)$. Such computation is subject to an initial condition $\mathbf{h}_k(t_s)=\psi(\mathbf{h}_k^{i-1}(t_e), \mathbf{x}_k(i))$ that includes the node representations computed in the previous sub-problem and the current node input state. In the bottom right, the discretized solution of the ODE is computed as iterative steps of the method over a discrete set of points in the time interval $[t_s, t_e]$.}
\label{fig:method}
\vspace{-2pt}
\end{figure*}

We now proceed to derive the condition under which the ODE is constrained to the stable and non-dissipative behavior, allowing for the propagation of long-range dependencies in the information flow. We start by defining the concepts of non-dissipativeness\footnote{The reader is referred to \citep{glendinning_1994, stabilityODE} for an in-depth analysis of dissipative dynamical systems.} as follow
\begin{definition}[Non-dissipativeness over a C-TDG]
Let $u,v\in\mathcal{V}(t)$ be two nodes of the C-TDG at some time $t$, connected by a path of length $L$. If an event $o_i$ occurs at node $u$, then the information of $o_i$ is propagated from $u$ to $v$, $\forall L\geq0$.
\end{definition}

We start by instantiating Eq.~\ref{eq:ode} as 
\begin{equation}
\resizebox{0.43\textwidth}{!}{$
\label{eq:our_ode}
\frac{\partial \mathbf{h}_u(t)}{\partial t} = \sigma \Bigl(\mathbf{W}_t \mathbf{h}_u(t) 
     +\Phi\left(\{\mathbf{h}_v(t),\mathbf{e}_{uv}, t_v^-, t \}_{v\in\mathcal{N}_u^t}\right) \Bigr)
$}
\end{equation}
where $\sigma$ is a monotonically non-decreasing activation function; $\Phi$ is the aggregation function that computes the representation of the neighborhood of the node $u$ considering node states and edge features; $t_v^-$ is the time point of the previous event for node $v$; and  $\mathbf{W}_t\in\mathbb{R}^{d\times d}$. We notice that including $t_v^-$ in $\Phi$ has the role of encoding the time elapsed since the previous event involving node $v$. This represents a force that may smoothly update the node’s current state during the time interval to prevent the staleness problem~\citep{dynamicgraph_survey}.

As discussed in \cite{StableArchitecture} and \cite{gravina2023antisymmetric}, a non-dissipative propagation is directly linked to the sensitivity of the solution of the ODE to its initial condition, thus to the stability of the system. Such sensitivity is controlled by the Jacobian's eigenvalues of Eq.~\ref{eq:our_ode}. Given $\lambda_i(\mathbf{J}(t))$ the $i$-th eigenvalue of the Jacobian, when $\max_{i=1,...,d} Re(\lambda_i(\mathbf{J}(t))) > 0$, a small perturbation of the initial condition would cause an exponentially exploding difference in the nodes representations, and the system would be unstable.
On the contrary, for 
$\max_{i=1,...,d} Re(\lambda_i(\mathbf{J}(t))) \ll 0$, 
the difference in the node representations would vanish exponentially fast over time, thereby making the node representations insensitive to differences in the initial condition. This results in a lossy system in which only local neighborhood information is preserved, while long-range dependencies among nodes are forgotten. Consequently, the resulting system is dissipative. Lastly, if $Re(\lambda_i(\mathbf{J}(t))) = 0$ for $i=1,...,d$ the initial condition is effectively propagated into the final node representation, making the system both stable and non-dissipative\footnote{This result holds also when the eigenvalues of the resulting Jacobian are still bounded in a small neighborhood around the imaginary axis~\citep{gravina2023antisymmetric}.}. The next proposition ensures that the employment of anti-symmetric weight matrices constrains the Jacobian's eigenvalues to be imaginary, allowing a stable and non-dissipative behavior of the ODE in Eq.~\ref{eq:our_ode}. 
\begin{proposition}\label{prop:imaginary_eigenvalues}
Provided that the weight matrix $\mathbf{W_t}$ is anti-symmetric\footnote{A matrix $\mathbf{M}\in\mathbb{R}^{d\times d}$ is anti-symmetric if $\mathbf{M}^\top = -\mathbf{M}$.} and the aggregation function $\Phi$ does not depend on $\mathbf{h}_u(t)$, the Jacobian matrix resulting from the ODE in Eq.~\ref{eq:our_ode} has purely imaginary eigenvalues, \ie $$Re(\lambda_i(\mathbf{J}(t))) = 0, \forall i=1, ..., d.$$
\end{proposition}
See proof in Appendix~\ref{app:imaginary_eigenvalues}.
\revise{We provide a more in-depth analysis of non-dissipativeness over time in Appendix~\ref{app:temporal_analysis}, showing when \adgn is both non-dissipative over space and time.}

Now that we have defined the conditions under which the ODE in Eq.~\ref{eq:our_ode} is stable and non-dissipative, \ie it can propagate long-range dependencies between nodes in the C-TDG, we observe that computing the analytical solution of an ODE is usually infeasible. It is common practice to rely on a discretization method to compute an approximate solution by multiple applications of the method over a discrete set of points in the time interval $[t_s, t_e]$. This process is visually summarized at the bottom of Figure~\ref{fig:method}. We employ the \textit{forward Euler's method} to discretize Eq.~\ref{eq:our_ode} for the $i$-th Cauchy sub-problem, yielding the following node state update equation for the node $u$ at step $\ell$:
% \begin{equation}\label{eq:discretization}
%     \mathbf{h}^{\ell}_u = \mathbf{h}^{\ell-1}_u +\epsilon \sigma \left((\mathbf{W}_\ell-\mathbf{W}_\ell^\top-\gamma\mathbf{I})\mathbf{h}^{\ell-1}_u + 
%     \Phi\left(\{\mathbf{h}_v(t),\mathbf{e}_{uv}, t_v^-, t \}_{v\in\mathcal{N}_u^t}\right)%\Phi(\mathbf{H}^{\ell-1},\mathbf{E}, \mathcal{N}_u^t) + \mathbf{V}_\ell (\mathbf{t}- \mathbf{t}^-_u) 
%     + \mathbf{b}_\ell \right),
% \end{equation}
\begin{multline}\label{eq:discretization}
    \mathbf{h}^{\ell}_u = \mathbf{h}^{\ell-1}_u +\epsilon \sigma \Bigl((\mathbf{W}_\ell-\mathbf{W}_\ell^\top-\gamma\mathbf{I})\mathbf{h}^{\ell-1}_u + \\
    +\Phi\left(\{\mathbf{h}_v(t),\mathbf{e}_{uv}, t_v^-, t \}_{v\in\mathcal{N}_u^t}\right) \Bigr),
\end{multline}
with $\epsilon>0$ being the discretization step size.
We notice that the anti-symmetric weight matrix $(\mathbf{W}_\ell-\mathbf{W}_\ell^\top)$ is subtracted by the term $\gamma\mathbf{I}$ to preserve the stability of the forward Euler's method, see Appendix~\ref{app:euler_stability} for a more in-depth analysis. We refer to $\mathbf{I}$ as the identity matrix and $\gamma$ to a hyper-parameter that regulates the stability of the discretized diffusion. We note that the resulting neural architecture contains as many layers as the discretization steps, \ie $L = t_e/\epsilon$.

As previously discussed for the ODE, the number of iterations in the discretization (i.e., the terminal time $t_e$) plays a crucial role in the propagation. Specifically, few iterations result in a localized event propagation. Consequently, the non-dissipative event propagation does not reach each node in the graph, causing a \textit{truncated} non-dissipative propagation. This method allows scaling the radius of propagation of information depending on the number of discretization steps, thus allowing for a scalable long-range propagation in C-TDGs. Crucially, we notice that, even with few discretization steps, it is still possible to propagate information from a node $u$ to $z$ (if a path of length $P$ connects $u$ and $z$). As an example, consider the situation depicted in the left segment of Figure~\ref{fig:method}, where nodes $u$ and $v$ establish a connection at some time $t$, and our objective is to transmit this information to node $z$. In this scenario, we assume $L=1$, thus the propagation is truncated before $z$. Upon the arrival of the %initial event
event at time $t$, this is initially relayed (due to the constraint of $L=1$) to node $k$, which then captures and retains this information. If a future event at time $t+\tau$ involving node $k$ occurs, its state is propagated, ultimately reaching node $z$. Consequently, the information originating from node $u$ successfully traverses the structure to reach node $z$. 
More formally, if it exists a sequence of (at least $P/L$) successive events, such that each future $i$-th event is propagated to an intermediate node at distance $iP/L$ from $u$, then $u$ is able to directly share its information with $z$. 
Therefore, even with a limited number of discretization steps, the non-dissipative behavior enables scaling the single event propagation to cover a larger portion of the C-TDG.
We also notice that if the number of iterations is at least equal to the longest shortest path in the C-TDG, then each event is always propagated throughout the whole graph. 

We name the overall framework defined above \fulladgn (\adgn). Note that $\Phi$ in Eq.~\ref{eq:our_ode} and \ref{eq:discretization} can be any function that aggregates nodes and edges states. Then, \adgn can leverage the aggregation function that is more adequate for the specific task. As an exemplification of this, in Section~\ref{sec:experiments} we leverage the aggregation scheme based on the one proposed by \cite{TrasformerConv}:
% \begin{equation}\label{eq:aggregation}
%     \Phi\left(\{\mathbf{h}_v(t),\mathbf{e}_{uv}, t_v^-, t \}_{v\in\mathcal{N}_u^t}\right) =
% \sum_{v \in \mathcal{N}_u^t \cup \{ u \}} \alpha_{uv} \left(\mathbf{V}_n\mathbf{h}_{v}^{\ell-1} + \mathbf{V}_e\hat{\mathbf{e}}_{uv}\right)
% \end{equation}
\begin{multline}\label{eq:aggregation}
    \Phi\left(\{\mathbf{h}_v(t),\mathbf{e}_{uv}, t_v^-, t \}_{v\in\mathcal{N}_u^t}\right) =\\
=\sum_{v \in \mathcal{N}_u^t \cup \{ u \}} \alpha_{uv} \left(\mathbf{V}_n\mathbf{h}_{v}^{\ell-1} + \mathbf{V}_e\hat{\mathbf{e}}_{uv}\right)
\end{multline}
where $\hat{\mathbf{e}}_{uv} = \mathbf{e}_{uv} \| \left(\mathbf{V}(t-t_v^-)\right)$ is the new edge representation computed as the concatenation between the original edge attributes and a learned embedding of the elapsed time from the previous neighbor interaction, and $\alpha_{uv}=\textrm{softmax} \left(\frac{\mathbf{q}^{\top}\mathbf{K}}{\sqrt{d}} \right)$ is the attention coefficient 
with $d$ the hidden size of each head, $\mathbf{q} = \mathbf{V}_q\mathbf{h}_u^{\ell-1}$, and $\mathbf{K} = \mathbf{V}_k\mathbf{h}_v^{\ell-1} + \mathbf{V}_e\hat{\mathbf{e}}_{uv}$. We use $\left(\mathbf{V}(t-t_v^-)\right)$ as a force that smoothly updates the node’s current state to prevent the staleness problem.


Despite \adgn being designed from the general perspective of layer-dependent weights, it can also be be used with weight sharing between layers, which we use throughout Section~\ref{sec:experiments}.


==> tables/config_link_pred.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.15}
\caption{The grid of hyper-parameters employed during model selection in the link prediction task. The best configuration of each model is run 5 times with different random seeds for multiple weight initializations. Models have a maximum number of learnable parameters of $\sim$140k. Training is run for 1000 epochs and early stopping with a patience of 50 epochs on the validation score. Neighbor sampler size is 5, and batch size is 256. The optimized metric is the AUC on the validation set. 
Memory dim and DGN dim are the same in the architecture.\\\label{tab:configs_link_pred}}
\centering
\footnotesize
\begin{tabular}{l|l}
\hline\toprule 
 & \textbf{Configs}\\\midrule %\hline
optimizer & Adam\\%\hline
learning rate & $10^{-4}$, $10^{-5}$\\%\hline
weight decay & $10^{-6}$\\%\hline
n. GCLs & 1, 3, 5 \\%\hline
$\sigma$ & tanh\\%\hline
$\epsilon$ & 0.5, $10^{-1}$, $10^{-2}$, $10^{-3}$\\%\hline
$\gamma$ &  0.5, $10^{-1}$, $10^{-2}$, $10^{-3}$\\%\hline
$\psi$ & concat, $\psi = \text{tanh}(\textbf{h}^{i-1}(t_e)||\mathbf{x}(i))$\\
time dim & 16\\\midrule %\hline
\multirow{5}{3cm}{memory dim and DGN dim} & TGN: 33, 20\\
& DyRep: 118, 87\\
& JODIE: 164, 122\\
& TGAT: 33, 23 \\ 
& \adgn: 128, 96\\
\bottomrule\hline
\end{tabular}
\end{table}

==> tables/config_pascal_voc.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.15}
\caption{The grid of hyper-parameters employed during model selection in the \texttt{temporal Pascal-VOC} task. Each configuration is run 5 times with different random seeds for multiple weight initializations. Models have a maximum number of learnable parameters of $\sim$40k. Training is run for 200 epochs. We use a learning rate scheduler which halves the learning rate with a patience of 20. Neighbor sampler size is 5, and batch size is 256. The optimized metric is the F1-score on the validation set. Memory dim and DGN dim are the same in the architecture.\\\label{tab:configs_pascal_voc}}
\centering
\footnotesize
\begin{tabular}{l|l}
\hline\toprule
 & \textbf{Configs}\\\midrule %\hline
optimizer & Adam\\%\hline
learning rate & $3\cdot10^{-4}$\\%\hline
weight decay & $10^{-5}$\\%\hline
n. GCLs & 1, 3, 5 \\%\hline
$\sigma$ & tanh\\%\hline
$\epsilon$ & 1, 0.5, $10^{-1}$, $10^{-2}$\\%\hline
$\gamma$ & 1, 0.5, $10^{-1}$, $10^{-2}$\\%\hline
$\psi$ & concat, $\psi = \text{tanh}(\textbf{h}^{i-1}(t_e)||\mathbf{x}(i))$\\
time dim & 1\\\midrule %\hline
\multirow{5}{3cm}{memory dim and DGN dim} & TGN: 21, 10\\
& DyRep: 74, 37\\
& JODIE: 97, 48\\
& TGAT: 24, 12 \\ 
& \adgn: 74, 37\\
\bottomrule\hline 
\end{tabular}
\end{table}


==> tables/config_seq_class.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.15}
\caption{The grid of hyper-parameters employed during model selection in the sequence classification task. Each configuration is run 10 times with different random seeds for multiple weight initializations. Models have a maximum number of learnable parameters of $\sim$20k. Training is run for 20 epochs. We use a learning rate scheduler which halves the learning rate with a patience of 5. Neighbor sampler size is 5, and batch size is 128. The optimized metric is the loss on the validation set. Memory dim and DGN dim are the same in the architecture.\\\label{tab:configs_seq_class}}
\centering
\footnotesize
\begin{tabular}{l|l}
\hline\toprule %\hline\hline
 & \textbf{Configs}\\\midrule%\hline
optimizer & Adam\\%\hline
learning rate & $3\cdot10^{-4}$\\%\hline
weight decay & $10^{-7}$\\%\hline
n. GCLs & 1, 3, 5 \\%\hline
$\sigma$ & tanh\\%\hline
$\epsilon$ & 1, 0.5, $10^{-1}$, $10^{-2}$\\%\hline
$\gamma$ & 1, 0.5, $10^{-1}$, $10^{-2}$\\%\hline
$\psi$ & concat, $\psi = \text{tanh}(\textbf{h}^{i-1}(t_e)||\mathbf{x}(i))$\\
time dim & 1\\\midrule %\hline
\multirow{5}{3cm}{memory dim and DGN dim} & TGN: 19, 9\\
& DyRep: 53, 26\\
& JODIE: 69, 34\\
%& \revise{TGAT: 24, 12} re-run this? \\ 
& TGAT: 24, 12 \\ 
& \adgn: 53, 26\\
\bottomrule\hline%\hline\hline
\end{tabular}
\end{table}

